Technical Language Processing for Telecommunications Specifications

Large Language Models (LLMs) are continuously being applied in a more diverse set of contexts. At their current state, however, even state-of-the-art LLMs such as Generative Pre-Trained Transformer 4 (GTP-4) have challenges when extracting information from real-world technical documentation without a heavy preprocessing. One such area with real-world technical documentation is telecommunications engineering, which could greatly benefit from domain-specific LLMs. The unique format and overall structure of telecommunications internal specifications differs greatly from standard English and thus it is evident that the application of out-of-the-box Natural Language Processing (NLP) tools is not a viable option. In this article, we outline the limitations of out-of-the-box NLP tools for processing technical information generated by telecommunications experts, and expand the concept of Technical Language Processing (TLP) to the telecommunication domain. Additionally, we explore the effect of domain-specific LLMs in the work of Specification Engineers, emphasizing the potential benefits of adopting domain-specific LLMs to speed up the training of experts in different telecommunications fields.

==> 99-future.tex <==

(just for us, not for this) The contribution in the second paper

\begin{enumerate}
    \item (1) Evaluation of NLP/LLM methodologies for responding to the common questions in Telecom Specs
    \item (2) methods: [1]: (baseline; no adjustments), [2]: in-context learning / few-shot prompting, [3] : retrieval augmented generation
    \item (3) models: closed-source (e.g. GPT-x?) / open models (LLaMax, Mixtral..)
    \item (4) approach: "single query" vs. "agent-based"
\end{enumerate}



(just for us, not for this) The contribution in the third paper

\begin{enumerate}
    \item user evaluation
    \item helping users understand the need to define metadata
    \item helping users write documents in a certain way
    
\end{enumerate}



(just for us, not for this) The contribution in a subsequent paper

\begin{enumerate}
    \item leverage LLMs for assessing whether internal specifications have written in a sufficient manner
    
\end{enumerate}

